Learning to Project for Cross-Task Knowledge Distillation

Traditional knowledge distillation (KD) relies on a proficient teacher trained on the target task, which is not always available. In this setting, cross-task distillation can be used, enabling the use of any teacher model trained on a different task. However, many KD methods prove ineffective when applied to this cross-task setting. To address this limitation, we propose a simple modification: the use of an inverted projection. We show that this drop-in replacement for a standard projector is effective by learning to disregard any task-specific features which might degrade the student's performance. We find that this simple modification is sufficient for extending many KD methods to the cross-task setting, where the teacher and student tasks can be very different. In doing so, we obtain up to a 1.9% improvement in the cross-task setting compared to the traditional projection, at no additional cost. Our method can obtain significant performance improvements (up to 7%) when using even a randomly-initialised teacher on various tasks such as depth estimation, image translation, and semantic segmentation, despite the lack of any learned knowledge to transfer. To provide conceptual and analytical insights into this result, we show that using an inverted projection allows the distillation loss to be decomposed into a knowledge transfer and a spectral regularisation component. Through this analysis we are additionally able to propose a novel regularisation loss that allows teacher-free distillation, enabling performance improvements of up to 8.57% on ImageNet with no additional training costs.

==> figures/depth-size-vs-performance-same-to-cross-task.tex <==
\begin{figure}[t]
    \centering
    \subfigure[Depth $\rightarrow$ Depth]{\includegraphics[width=.32\textwidth]{figures/Depth_params_v2.png}}
    \subfigure[Insseg $\rightarrow$ Depth]{\includegraphics[width=.32\textwidth]{figures/Insseg_params_v2.png}}
    \subfigure[Random $\rightarrow$ Depth]{\includegraphics[width=.32\textwidth]{figures/Random_params_v2.png}}
    \vspace{1em}
    \caption{\textbf{Comparing performance of different-sized depth students} with both the traditional projection and our novel inverted projection.
    Where there is knowledge to transfer from teacher to student (i.e. the two tasks are similar), the traditional projection performs better, but when the teacher is random, the opposite is true. Only decoder size is varied. A MobileNetV2 \cite{Fox2018MobileNetV2:Bottlenecks} is used as the backbone.}
    \label{fig:params_vs_performances}
\end{figure}


==> tables/manual_reg.tex <==
\begin{table}
    \centering
    \footnotesize
    \begin{tabular}{lccc}
        \toprule
        \belowrulesepcolor{mygrey}
        \rowcolor{mygrey} Method & RMS $\downarrow$ & Abs $\downarrow$ & $\delta_1$ $\uparrow$ \\
        \aboverulesepcolor{mygrey}
        \midrule
        \textit{(Baseline) AiT (SwinV2-B) \cite{ning_all_2023}} & \textit{0.365}            & \textit{0.105}            & \textit{0.907}                 \\
        \midrule
         $\mathcal{L}_{spectral}$ $(r = 1)$              & 0.352            & 0.105            & 0.902                 \\
         $\mathcal{L}_{spectral}$ $(r = 2)$              & \textbf{0.340}   & \textbf{0.096}   & \textbf{0.914}        \\
         $\mathcal{L}_{spectral}$ $(r = 4)$              & 0.349            & 0.099            & 0.911                 \\
         $\mathcal{L}_{spectral}$ $(r = 8)$              & 0.344            & \textbf{0.096}   & 0.910                 \\
         $\mathcal{L}_{spectral}$ $(r = 16)$             & 0.348            & 0.098            & 0.912                 \\
         $\mathcal{L}_{spectral}$ $(r = 32)$             & 0.347            & 0.100            & 0.909                 \\
        \bottomrule
    \end{tabular}
    \vspace{1em}
    \caption{\textbf{Teacher-free distillation} using our spectral regularisation loss on the NYUv2 dataset using AiT \cite{ning_all_2023} on a SwinV2-b base. The regularisation loss is generally robust to different values of $r$, with $r = 2$ being optimal.
    }
    \label{tab:manual-reg-ait}
\end{table}


==> tables/rebuttal/class-depth-enb0-rn50.tex <==
\begin{table}[t]
\centering
\scriptsize
\resizebox{1\textwidth}{!}{
\begin{tabularx}{\textwidth}{XX|ccc|ccc}
\toprule
\belowrulesepcolor{mygrey}
\rowcolor{mygrey} \multicolumn{2}{r|}{Student Arch (backbone) $\longrightarrow$} &
  \multicolumn{3}{c|}{EfficientNet-B0 (5.3M)} &
  \multicolumn{3}{c}{ResNet-50 (25.6M)} \\
\rowcolor{mygrey} KD Method &
  Projection type &
  $\delta_1 \uparrow$ &
  Abs. $\downarrow$ &
  RMS $\downarrow$ &
  $\delta_1 \uparrow$ &
  Abs. $\downarrow$ &
  RMS $\downarrow$ \\ 
\aboverulesepcolor{mygrey}  
\midrule
\textit{None (baseline)} &
  \textit{N/A} &
  0.845 &
  0.127 &
  0.440 &
  0.811 &
  0.144 &
  0.480 \\ \midrule
AT~\cite{Zagoruyko2019PayingTransfer} &
  Original &
  0.850 &
  0.125 &
  0.433 &
  0.814 &
  \textbf{0.143} &
  0.477 \\
 &
  Inverted (ours) &
  \textbf{0.853} &
  \textbf{0.123} &
  \textbf{0.430} &
  \textbf{0.816} &
  \textbf{0.143} &
  \textbf{0.475} \\
 &
  \textit{Improvement} &
  \cellcolor[HTML]{F3FFF3}\textit{0.35\%} &
  \cellcolor[HTML]{C5FFC5}\textit{1.61\%} &
  \cellcolor[HTML]{E3FFE3}\textit{0.79\%} &
  \cellcolor[HTML]{F6FFF6}\textit{0.26\%} &
  \cellcolor[HTML]{FAFFFA}\textit{0.14\%} &
  \cellcolor[HTML]{F2FFF2}\textit{0.38\%} \\ \midrule
PKT~\cite{Passalis2018LearningTransfer} &
  Original &
  0.851 &
  0.124 &
  0.432 &
  0.816 &
  0.143 &
  0.473 \\
 &
  Inverted (ours) &
  \textbf{0.853} &
  \textbf{0.123} &
  \textbf{0.431} &
  \textbf{0.821} &
  \textbf{0.141} &
  \textbf{0.470} \\
 &
  \textit{Improvement} &
  \cellcolor[HTML]{F7FFF7}\textit{0.25\%} &
  \cellcolor[HTML]{D1FFD1}\textit{1.29\%} &
  \cellcolor[HTML]{F5FFF5}\textit{0.30\%} &
  \cellcolor[HTML]{E9FFE9}\textit{0.63\%} &
  \cellcolor[HTML]{D4FFD4}\textit{1.19\%} &
  \cellcolor[HTML]{E6FFE6}\textit{0.70\%} \\ \midrule
FitNets~\cite{romero_fitnets_2015} &
  Original &
  0.845 &
  0.125 &
  0.439 &
  0.812 &
  0.145 &
  0.480 \\
 &
  Inverted (ours) &
  \textbf{0.850} &
  \textbf{0.124} &
  \textbf{0.434} &
  \textbf{0.813} &
  \textbf{0.142} &
  \textbf{0.476} \\
 &
  \textit{Improvement} &
  \cellcolor[HTML]{EDFFED}\textit{0.50\%} &
  \cellcolor[HTML]{ECFFEC}\textit{0.53\%} &
  \cellcolor[HTML]{CFFFCF}\textit{1.34\%} &
  \cellcolor[HTML]{FAFFFA}\textit{0.16\%} &
  \cellcolor[HTML]{B9FFB9}\textit{1.93\%} &
  \cellcolor[HTML]{E3FFE3}\textit{0.77\%} \\ \bottomrule
\end{tabularx}%
}
\vspace{1em}
\caption{\textbf{Comparisons with different architecture pairs.} All experiments perform cross-task distillation from a classification teacher to a depth estimation student. The inverted projection is effective across various student model sizes and with different KD methods in this cross-task setting.}
\label{tab:rebuttal:enetb0-rn50-class2depth}
\end{table}

